ReFeed: Multi-dimensional Summarization Refinement with Reflective Reasoning on Feedback

Summarization refinement faces challenges when extending to multi-dimension. In this paper, we introduce ReFeed, a powerful summarization refinement pipeline that enhances multiple dimensions through reflective reasoning on feedback. To achieve this, we release SumFeed-CoT, a large-scale Long-CoT-based dataset optimized for training a lightweight model with reflective reasoning. Our experiments reveal how the number of dimensions, feedback exposure, and reasoning policy influence refinement performance, highlighting reflective reasoning and simultaneously addressing multiple feedback is crucial to mitigate trade-off between dimensions. Furthermore, ReFeed is robust to noisy feedback and feedback order. Lastly, our finding emphasizes that creating data with a proper goal and guideline constitutes a fundamental pillar of effective reasoning. The dataset and model will be released.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> section/legacy/1-intro-legacy.tex <==
\section{Introduction}

In text summarization, large language models (LLMs) have primarily aimed to enhance the faithfulness by incorporating more advanced methodologies, such as SYNFAC-EDIT 
and CPO \cite{mishra2024synfac,feng2024improving}. However, this emphasis on a single dimension, such as faithfulness, raise an important question: \emph{
Does improving only one dimension come at the cost of other aspects of summarization?"}
%This raises another important question: \emph{"whether improving only one dimension, such as faithfulness, involves a trade-off with other dimentions."} 
Generally, aligning model's responses with a single aspect often compromise other crucial aspects of quality \cite{guo2024controllable, song2024learning}. In light of these conflicts, it becomes important to enhance LLM's responses from a multi-dimensional perspective. Yet, effectively improving all dimension remains challenging not only because collecting multifaceted data is costly \cite{song2024learning} but also optimizing multi-dimension is complex \cite{ryu2024multi}.

One potential pathway is to apply \emph{post-hoc refinement} to the initial response, which can yield remarkable gains across various tasks \cite{madaan2024self, pan2024automatically}. Text refinement offers advantages in both cost efficiency and domain generalization \cite{cai2024ceret} compared to supervised fine-tuning (SFT) for summarization models, which require substantial amounts of human-annotated training data for each domain and dimension.
Moreover, this technique is further enhanced by incorporating external feedback generated by LLMs. \cite{liu2023improving, wadhwa2024learning, wan2024acueval}. Given that feedback can be easily configured as multifaceted through prompt engineering \cite{madaan2024self}, the refinement has the potential to be extended for multiple desired dimensions with external feedback.
% with external feedback tailored to the desired dimension
% Although, when taking into account these advantages, providing external feedback tailored to the desired dimension has the potential to extend to multiple dimensions, the current approach is focusing primarily on faithfulness and overlooking the trade-offs in a multi-dimensional perspective. 


%%%%%%%% Framework

\pdfcompresslevel=0
\pdfobjcompresslevel=0
\pdfminorversion=5

\begin{figure*}[t!]
\begin{center}
\includegraphics[width=16cm]{section/figure/refeed-overview.pdf}
% \vspace*{-0.5cm} % 하단 여백 추가
\end{center}
\vspace*{-0.5cm}
\caption{Overview of \algname{}. Each color indicates feedback related to its matching dimension}
\label{fig:overview}
\vspace*{-0.45cm}
\end{figure*}
%%%%%%%%%%%%%

However, extending refinement methods beyond a single dimension presents several challenges that must be addressed to be sufficient for multi-dimension. 
Firstly, multi-dimensional refinement must account for the \emph{trade-off} across various dimensions. What may be a correct refinement for one dimension could, in fact, be the result of sacrificing another dimension. Secondly, there exists a \emph{ordering bias}. Similar to training paradigms, multi-dimensional refinement can be approached in two main ways: "sequential," where each prompt addresses one dimension at a time, or "simultaneous," a single prompt with aggregating across all dimensions. Depending on the approaches, the refine model may  exhibit a preference for the specific positioning of dimensions within the prompt \cite{zhang2024batch} or prioritize subsequent feedback. Lastly, external feedback, derived from LLM evaluations on text, may exhibit deficiencies such as low accuracy or insufficient robustness, stemming from latent biases across various domains and models \cite{wang2023large, ye2023flask}. This defective feedback can be characterized as \emph{noisy feedback}. Although, refinement models are designed to be responsive to external feedback, assuming feedback is accurate, incorporating such noisy feedback may unintentionally affect both the target dimension and other aspects.

In this paper, we address the three challenges by proposing \textbf{\algname{}} 
 (\underline{\textbf{Re}}finement with \underline{\textbf{Re}}flective \underline{\textbf{Re}}asoning on \textbf{\underline{Feed}}back), specifically focusing on refining summaries by emphasizing three key dimensions: {faithfulness}, {completeness}, and {conciseness}\footnote{Recent studies emphasize that a human-preferred summary should be factually correct (faithfulness), include all key information (completeness), and avoid any irrelevant content (conciseness) \cite{song2024finesure, tang2024tofueval}.}. Our approach distills reasoning from models such as OpenAI's o1 \cite{jaech2024openai} and integrates \emph{reflective} reasoning on feedback into the refinement pipeline. Reasoning models like o1 exhibit reflective reasoning through \emph{long chain-of-thought} (Long-CoT). Its thinking process involves "backtracking," where in the model identifies mistakes and restarts its reasoning. \cite{wu2024comparative, zhong2024evaluation}. This has the potential to revisit feedback incorporation when trade-offs emerge during refinement, simultaneously handling of multiple dimensions. Furthermore, reflective reasoning enables a critical analysis of feedback, allowing for continuous validation of its correctness by tracing back through the reasoning process rather than adopting a receptive stance. Yet, given the high computational cost of such reasoning models, distilling this capability into smaller models presents a promising direction.

As shown in Figure \ref{fig:overview}, we first construct a large-scale dataset to enable complex reasoning in LLMs. Our dataset includes high-quality LLMs' reflective reasoning on feedback across three approaches: (1) backtracking to resolve trade-offs during the refinement; (2) adopting to simultaneous-style refinement on multi-dimensions; and (3) validating feedback to filter out noise. We utilize reflective reasoning data from a reasoning model, and then curate only well-structured and successful reasoning on feedback for refinement on summaries. 
Lastly, we train a model on the constructed dataset, where input feedback undergoes shuffled permutations across multiple dimensions to better mitigate order bias. We further perform a comprehensive analysis to identify which refinement pipeline, including prior two approaches, DCR \cite{wadhwa2024learning} and ACUEval \cite{wan2024acueval}, achieves a balanced improvement across multi-dimensions mitigating trade-offs, and maintains robustness in the presence of order bias and noisy feedback.

Our main contributions are: (1) We propose \textsc{\algname{}}, a multi-dimensional refinement pipeline that utilize reflective reasoning to address trade-offs, ordering bias, and noise, and develop light-weight models for this. 
(2) We release SumFeed-CoT, a large-scale dataset that captures Long-CoT reasoning on feedback, enabling successful refinement, even in the presence of noise and regardless of the order of dimension; and (3) We analyze the impact of five refinement pipeline, highlighting the trade-offs that arise when focusing on a single dimension and the vulnerabilities to order bias and noisy feedback.

%s—including previous refinement approach on single dimension—
\label{sec:introduction}



==> section/legacy/3-method-legacy.tex <==
% \vspace*{-0.1cm}
\section{Preliminary: Refinement Pipeline}
\label{sec:preliminary}

\newcolumntype{L}[1]{>{\raggedright\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{X}[1]{>{\centering\let\newline\\\arraybackslash\hspace{0pt}}p{#1}}


\subsection{Refinement Modules}
In general, the text refinement pipeline involves three key modules, namely detection, reasoning, and refinement models \cite{wadhwa2024learning}.% We overview each module below.

\paragraph{Detection Model.} This employs automated evaluators like Minicheck \cite{tang2024minicheck} to pinpoint the parts requiring revision, such as sentences or atomic facts, using binary labels. Notably, binary labels alone can drive effective refinements \cite{wan2024acueval, wadhwa2024learning}, making the detect label itself a form of feedback. We thus treat detect labels as feedback in this work.

\paragraph{Reasoning~(Critique) Model.} This generates specific reason why correction is need and suggest how to fix. It is often used sequentially after the detection module \cite{wadhwa2024learning} or concurrently with it \cite{song2024finesure}. Feedback can thus be generated by either a single module (detection or reasoning) or by critique based on detect labels. While such step is referred to as "critique," in this work, we instead refer to it as "reasoning" to better represent their role.
% While it can operate independently \cite{madaan2024self}, 

\paragraph{Refinement Model.} This refines text either without feedback or with provided feedback. Refinement is generally more effective when feedback is available rather than when performed directly without it. In such cases, the quality of the feedback plays a crucial role in determining the effectiveness of the refinement outcome.

\subsection{Extension to Multi-Dimension}

We introduce three key aspects, A1–A3, that are essential for designing a refinement pipeline across multiple dimensions.

\paragraph{A1: Trade-off in Multi-Feedback.}
Reasoning and refinement models should reconcile the feedback derived from {multiple} detect models to address multiple dimensions, thereby making each feedback component interdependent with the others. %In such dependent settings, prompts for LLMs include the definitions or feedback for each dimension. 
Dependency here can act as constraints similar to multi-objective optimization \cite{guo2024controllable}. For instance, when addressing faithfulness and completeness at once, it is preferable to replace only erroneous phrases to preserve completeness, while deleting the entire sentence to fix a minor faithfulness issue. The latter is considered "{over-correction"} \cite{shridhar2024art}, leading to the loss of key information, which harm completeness. Therefore, considering trade-offs from interdependent multi-feedback is crucial in reasoning. 

% rather than removing a sentence entirely 
\vspace{-0.1cm}

\paragraph{A2: Sequential vs. Simultaneous.}
The refinement model can incorporate multi-dimensional feedback via two strategies inspired by training methodologies; "sequential" and 
"simultaneous." The sequential approach \cite{lou2024spo} provides feedback stepwise for each individual dimension, allowing concentrated attention on a target dimension that may yield higher gains. In contrast, the simultaneous approach \cite{wu2023fine, guo2024controllable} aggregates feedback across all dimensions into a single prompt. This ensures a more balanced consideration of all dimensions, though it lacks the concentrated attention as the sequential one.

\vspace{-0.1cm}

\paragraph{A3: Inaccurate Feedback.}
While reasoning and refinement models are designed {receptive reasoning} to feedback, it is important to note that LLM-generated feedback may be biased or inaccurate. Hence, LLMs' feedback may instead amplify flawed reasoning \cite{turpin2024language}. 
In this context, Long-CoT like OpenAI's o1 have gained attention for its ability to perform reflective reasoning. By iteratively reviewing feedback and retracing the reasoning, reflective reasoning can identify inaccurate feedback and mitigate the continuation of erroneous reasoning.

% In this regard, reasoning through "Long CoT" like OpenAI's o1 attracts attention for their capacity to engage in {reflective reasoning}. Its thinking process generally involves "backtracking," where in the model identifies mistakes and restarts its reasoning \cite{wu2024comparative}.

\subsection{Simple Pipeline for Multi-Dimension}
\label{sec:baseline}
We design five simple pipelines addressing three key aspects, all of which serve as baselines. 
%
We integrate reasoning and refinement into a single module, referred to as "reason+refine" for scalability: relying on textual feedback from specific reasoning model can lead to biases and limit the gain of refinement. In this pipeline, a document and its summary are first processed by a detection model. A reason+refine module then generate both a reasoning on feedback and a revised summary.

We introduce four baselines (P1--P4), each starting with single-dimension refinement and gradually integrating the three aspects from A1 to A3. 

\smallskip
\noindent\textbf{$\bullet$ P1:} This is the base pipeline designed specifically for single-dimension feedback, following "detect$\rightarrow$reason+refine" structure.


\smallskip
\noindent\textbf{$\bullet$ P2:} This extends P1 to support multi-dimensional feedback sequentially. The reason+refine model iterates three times, each using the improved summary from the previous run and integrating feedback for faithfulness, completeness, and conciseness in that order.


\smallskip
\noindent\textbf{$\bullet$ P3:} This is identical to P2, except for the prompt strategy. While P2 employs a single-turn prompt that resets the session at each step, P3 uses a multi-turn approach, retaining memory of previous runs for improved continuity.


\smallskip
\noindent\textbf{$\bullet$ P4:} Unlike P2 and P3, this shifts sequential prompting to a simultaneous approach, providing feedback for all three dimensions.

The detailed categorization of the four baselines are presented in the columns 1--5 of Table \ref{tab:exp1}.

% For the multi-dimensions, we adopt five pipelines that consider three key aspects. In our baseline, we combine the reasoning and refinement modules, which is refer as "reason+refine." In this pipeline, a document \(D\) and its summary \(S\) are first processed by a detection model \(M_D\), which identifies parts that need fixing in \(S\) and produces binary feedback \(F = M_D(S)\). A subsequent model then jointly performs reasoning and refinement to generate a pair \((R, S')\), where \(R\) is the reasoning on feedback and \(S'\) is the revised summary.
% This combination is motivated by scalability concerns: relying on textual feedback from a specific reasoning model leads to bias, as refinement becomes limited to that model's reasoning, thereby degrading scalability. 


%We first extend our single-dimension refinement pipeline (P1) to multiple dimensions by addressing multi-feedback dependencies (A1) using two approaches: P2 processes each dimension with a single-turn prompt, while P3 first defines all dimensions in prompt and then refines them sequentially via multi-turn prompts. Next, taking into account refinement strategies (A2), we transition from a sequential to a simultaneous refinement (P4). Finally, to better handle the noisy feedback (A3), we develop P4 by incorporating reflective reasoning, which is \algname{}. In this work, we explore these five pipelines in depth. See Appendix \ref{sec:appendix-refinement-details} for details on each pipeline and prompt. 

%%%%%%%%%%%% Table to explain configuration ##############

% \begin{table}[t]
% \begin{center}
% \footnotesize
% \begin{tabular}{|X{0.2cm} |X{0.82cm} |X{1.6cm} |X{1.73cm} |X{1.28cm}|} \toprule
% \!\!ID\!\! & Dim. & Feedback & Refinement & Reason \\ \midrule
% \!\!C1\!\! & Single & Independent  & Sequential & Receptive \\ 
% \!\!C2\!\! & Multi & Independent  & Sequential & Receptive \\ 
% \!\!C3\!\! & Multi & Dependent  & Sequential & Receptive \\ 
% \!\!C4\!\! & Multi & Dependent  & Simultaneous & Receptive \\ 
% \!\!C5\!\! & Multi & Dependent  & Simultaneous & Reflective \\ \bottomrule
% \end{tabular}
% \end{center}
% \vspace*{-0.3cm}
% \caption{Five different configurations for refinement on Multi-dimensions.}
% \label{tab:exp_configuration}
% \vspace*{-0.6cm}
% \end{table}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%% Framework

\begin{figure}[!t]
\includegraphics[width=1\linewidth]{example-image-a} \hfill
\vspace*{-0.5cm}
\caption{Training data generation: we collect high-quality reasoning data from reasoning model across two feedback quality by setting proper goal and guideline.}
\vspace*{-0.6cm}
\end{figure}

%%%%%%%%%%%%%


% \vspace*{-0.1cm}
\section{Re$^3$Feed: Reflective Refinement}
\label{sec:train-data-detail}
% \vspace*{-0.1cm}

\algname{} differs from the four baselines, resembling P4 (multi-dimension, simultaneous feedback) but uniquely integrating \emph{reflective} reasoning in refinement. To distill this capability, it includes data construction and a dedicated training process.
%We start by constructing a training dataset to fine-tune LLMs for multi-dimensional refinement using reflective reasoning. Then, we fine-tune Llama models to distill reasoning capabilities for summary refinement using the constructed dataset. 
Note that, in refinement, our focus is on enhancing the quality of the initial summary across three key dimensions \cite{song2024finesure, tang2024tofueval}: 

$\bullet$ \emph{Faithfulness} refers the factual consistency of the summary with its grounded document; 

$\bullet$ \emph{Completeness} refers the coverage of key information in the summary; and 

$\bullet$ \emph{Conciseness} refers to the succinctness of the summary, avoiding unnecessary details. 

We present the details of them in Appendix \ref{sec:appendix-summary-metric}.

\subsection{SumFeed-CoT Dataset}
Since existing reasoning models mainly trained on math and code generation, they exhibit some misalignment with the need of summarization refinement. 
Thus, we guide the teacher model to refine based on reflective reasoning on feedback, thereby constructing a training dataset. 

Upon prior work \cite{jaech2024openai, xu2025towards}, we construct our dataset through three key stages: \emph{goal specification}, \emph{guideline formulation}, and \emph{quality control}. A well-defined goal, such as a golden label, provides a clear reference for the reasoning model, steering it towards an optimal reasoning path. Detailed guidelines further reinforce this process by ensuring alignment between the reasoning trajectory and the intended objective \cite{jaech2024openai}. Finally, rigorous quality control is essential for curating high-quality reasoning data \cite{lu2024mathgenie}, which, in turn, enhances the ability of student models to engage in reflective reasoning.

% \begin{itemize} 
% \setlength{\itemindent}{-0.7em}
% \vspace*{-0.2cm}
% \item \textbf{Goal Setting}: Define the ideal target (e.g., the golden label) for the reasoning process. 
% \vspace*{-0.2cm}
% \item \textbf{Guideline Formulation}: Provide task-specific constraints to guide the teacher model toward generating optimal reasoning paths. 
% \vspace*{-0.2cm}
% \item \textbf{Quality Control}: Ensure that the reasoning data consistently meets proper format and exhibits successful reasoning. 
% \end{itemize}



\subsubsection{Initial Feedback Collection}

We generate initial feedback for reasoning using document-summary pairs. Following \citet{song2024learning}, we sample 200 documents from the train split of seven source datasets across diverse domains and generate summaries using 13 different language models to ensure diversity of summary conditions. Each summary is evaluated with binary labels that identify sentences to fix for faithfulness or conciseness, or missing key facts that should be added for completeness through LLM-based evaluator\footnote{We used the most recent automated evaluator tailored for summarization, FineSurE \cite{song2024finesure}.}. To accomodate various quality feedback, we adapt the backbone of the LLM-based evaluator using both LLaMA-3.1-8B (low quality) and -70B (high quality) models. We then map the binary labels from the automatic evaluator to corresponding sentences and key facts, each of which serves as feedback to the refinement model.

After filtering feedback's format errors, we obtain 29K \texttt{<document,summary,feedback>} triplets,  each serving as input to the reason+refine model for summary refinement. Refer to Appendix \ref{sec:appendix-data-detail} for details on source data and prompts.


% to mitigate bias toward a specific critique model. %To handle low-quality feedback, we use both 8B and 70B LLaMA 3.1 models. 

\subsubsection{Reflective Reasoning Collection}

Summary refinement currently lacks a clear goal and guidelines. To address this, we define the ideal summary as one that needs no further feedback and concisely captures all key facts. We also establish guidelines to address three key aspects of multi-dimensional refinement: (1) backtracking for trade-offs, (2) simultaneous style to avoid order bias, and (3) noise filtering. Lastly, we curates high-quality reasoning via two criteria: \emph{reasoning format filtering}, which retains Long-CoT without formatting errors, and \emph{verification-based filtering}, which ensures that the reasoning meets established quality standards. The reasoning collecton process in our dataset is detailed as follows:

%%%%%%%% IMPORTANT %%%%%%%%%%%%%%%

%%%%%%%% IMPORTANT %%%%%%%%%%%%%%%

\paragraph{Goal Specification.} 
We define the best summary as the one selected from those generated by the 13 summarizers during the feedback collection step.
For each document, the best one is the summary with high quality that only needs minimal feedback. Based on the initial feedback, we select the summary with the highest average across faithfulness, completeness, and conciseness as the best one.
%Specifically, this is the summary that achieves the highest average score across three dimensions, as determined by the collected initial feedback.

\paragraph{Reasoning with Guideline.} 
We define a guideline to distill reflective reasoning from a teacher LLM\footnote{We used QwQ-32B-preview model, which exhibits Long-CoT capabilities comparable to o1-mini.} for summary refinement. The reasoning is collected by providing \texttt{<document, summary, feedback,best summary>} as input to the teacher LLM, along with our well-formed guideline, to induce reflective reasoning.
The reasoning derives how to refine the given summary by referencing the best summary (goal) as a standard.

Specifically, the guideline prompts the teacher LLM to reason across multiple dimensions simultaneously, incorporating backtracking to manage trade-offs. Additionally, it encourages the model to analyze the best summary’s attributes, allowing it to better filter out noisy feedback in the input on completeness and conciseness. Yet, this does not enhance faithfulness critique. Thus, we introduce explicit factual error definitions, aiding more accurate faithfulness feedback assessment \cite{wadhwa2024learning}. See Appendix \ref{sec:appendix-reasoning-detail} for details.

%Reasoning is generated using \texttt{<document,summary,feedback,best summary>} inputs, with outputs segmented into reasoning and a revised summary. See Appendix \ref{sec:appendix-reasoning-detail} for details.

% We prompt the model to reason across all dimensions simultaneously, using backtracking when necessary to manage trade-off. We further guide the model to identify key content by examining the attributes of the best summary, thereby better filtering out noisy feedback on completeness and conciseness. However, it does not enhance the critique on faithfulness. To address this, we provide definitions of factual error types, which help the model more accurately assess faithfulness \cite{wadhwa2024learning}. We generate reasoning using input pairs in the form \texttt{<document, summary, feedback, best summary>}, segment the output into reasoning and a revised summary. See Appendix \ref{sec:appendix-reasoning-detail} for reasoning generation prompt.

\paragraph{Quality Control.}
We retain only samples with over 5K tokens in reasoning after removing malformed outputs,  ensuring format compliance and compatibility with the student model's token limit. Next, we conduct a validity check, a task of verifying the revised summary with the collected reasoning indeed meets the following criteria: (1) faithfulness = 1, completeness $\geq 0.5$, and conciseness $\geq 0.5$; and (2) $\triangle$score is $\geq 0$ across all dimensions, meaning that the revised summary must improve upon the previous one in every dimension.

%Next, we regenerate feedback-based score to collect only cases where the $\triangle$score is $\geq 0$ across all dimensions and the revised summary satisfies: faithfulness = 1, completeness $\geq 0.5$, and conciseness $\geq 0.5$. 
%We adopt the QwQ-32B-preview model, which exhibits long CoT capabilities comparable to o1-mini, to generate training data. 

As a result, our final dataset includes 7.7K samples. We also randomly shuffle the feedback's dimensions in dataset. The details of training data can be found in Appendix \ref{sec:appendix-train-data-detail}.


% The quality of reasoning data is influenced by three key factors: \emph{model selection}, choosing a teacher model capable of long CoT; \emph{reasoning format filtering}, retaining extended reasoning sequences without formatting errors; \emph{verification-based filtering}, keeping reasoning meeting quality criteria \cite{lu2024mathgenie, jaech2024openai, wang2024drt}. Given these considerations, we choose QwQ-32B-preview, which performs comparably to o1-mini\cite{}, as the teacher model. We generate reasoning using input pairs in the form \texttt{<document, summary, feedback, best summary>}, segment the output into reasoning and a revised summary. Next, we retain only samples with over 5K tokens in reasoning after removing malformed outputs. Lastly, We regenerate feedback-based score to collect only cases where the $\triangle$score is $\geq 0$ across all dimensions and the revised summary satisfies: faithfulness = 1, completeness $\geq 0.5$, and conciseness $\geq 0.5$. 
% Our final dataset includes 7.7K samples. To prevent the model from developing biases based on the ordering of input dimensions, we randomly shuffle the dimensions in the prompt. The details of our training data can be found in Appendix \ref{sec:appendix-train-data-detail}.



\subsection{Training Details}

We fine-tune Llama-3.1-8B-Instruct (student) using LoRA \cite{hu2022lora} and DeepSpeed (ZeRO-3) \cite{rasley2020deepspeed}. The user prompt follows the same format as in reasoning generation, excluding the best summary and error types as seen in below. See Appendix \ref{sec:appendix-training-detail} for other training details.
 % The model's response is structured using XML tags to clearly separate reasoning from the revised summary: \texttt{<think>reason</think><answer>revised summary</answer>} 
\begin{tcolorbox}[colback=gray!10, colframe=black, title=The Input/Output of \algname{} ]
    Input: <Document, Summary, Feedback> \\
    Output: \\
    <think> Reasoning </think> \\
    <answer> Revised Summary </answer>
\end{tcolorbox}

% customize system prompts to encourage reflective reasoning.


%%%%%%%%%%%%%%%%%%%%%%%%%%



% \paragraph{RQ3: How does noisy feedback affect its own and other dimensions?} We evaluate the impact of noisy feedback on multi-dimensional refinement by assessing its dependency on the detect model. This experiment aims not only to determine the extent to which performance depends on the detect model but also to investigate whether noise in one feedback adversely affects other dimensions. This analysis will also reveal whether errors in the detect step transfer to later steps and whether such errors can be effectively mitigated depending on the reasoning style.







% \paragraph{Dimension Orders} 


% \paragraph{Dimension Orders} 
% For RQ1 and RQ3, we maintained a fixed dimension order; faithfulness – completeness – conciseness. In contrast, for RQ2, we conducted five trials with shuffled dimension orders. In Trials 1, each data point is assigned a random permutation of three dimensions. For Trials 2-4, We fix the last positions for each of the three dimensions and rearrange remaining positions randomly. Appendix \ref{sec:appendix-experiment-detail-order} illustrates the distribution of the dimension orders within our experiment.

% In each refinement pipeline, we utilized identical feedback labels generated using the same prompt employed during the training phase. feedback generation was conducted using the LLaMA 3.1 series. We assume that the 8B model produces lower-quality labels based on the evaluation of agreement with human labels in previous research., whereas the 70B model yields higher-quality labels. For refinement, we also select the LLaMA 3.1 8B-Instruct model across all configurations where no fine-tuning was applied, except for DCR and C5, which are fine-tuned models. A detailed description of the refinement setup is provided in Appendix \ref{sec:appendix-experiment-detail}.

% %%%%%%%%%%%%%% Table for previous model (Ver 1 - 색깔 없는 버전) %%%%%%%%


==> section/legacy/4-evaluation-order-last.tex <==
% \vspace*{-0.1cm}
\section{Experiment Setup}
\label{sec:experiment}


All pipelines use identical feedback labels generated from the same feedback generation prompt in train phase: sentence-level labels for faithfulness and conciseness, and key fact-level labels for completeness, except ACLEval, which adopts atomic fact, which refer to non-decomposable facts within a sentence. We use the LLaMA 3.1 8B-Instruct for feedback generation. For refinement, we also select the same model without fine-tuning, except for C5 and DCR. We maintains a fixed order; faithfulness–completeness–conciseness.

\paragraph{Test Dataset}
We use UniSumEval \cite{lee2023unisumeval}, a benchmark dataset to evaluate three dimensions. This dataset includes challenging source documents spanning nine domains, where summaries are prone to contain factual error, as well as initial summaries by nine recent summarizer, including both non-LLMs and LLMs. Appendix \ref{sec:appendix-experiment-detail} shows the feedback quality based on test dataset and the distribution of the dimension orders in our experiment.

% Given its complexity, UniSumEval serves as a rigorous testbed for evaluating the capability of each refinement pipeline across diverse document and summary conditions.

% we assume the 8B model produces low-quality feedback with more noise label based on its evaluation of agreement with humans \cite{oh2024learning}. 

% To address it, we conducted four trials with shuffled orders, while we maintained a fixed order in other experiments; faithfulness–completeness–conciseness. In first trials, each data point is assigned a random permutation of three dimensions. For Trials 2-4, we fix the final position of each dimension, while the remaining positions is randomized. We use high-quality labels by LLaMA 3.1-70B Instruct, which are almost free of noise, ensuring that our analysis focuses on the impact of order bias.

% We compare refinement performance using low-quality detect labels against that obtained with high-quality labels. 


% We use UniSumEval \cite{lee2023unisumeval}, a benchmark dataset that includes hallucinatory texts across nine domains: News, Lifestyle, Report, Med lit, Sci-fi, Daily Life, Booking, Interview, and Meeting, covering both dialogue and non-dialogue formats as well as varying text lengths. In our experiments, we use these texts and their summaries, which generate nine recent summarization models: BART, Flan-T5, Phi-2, Mistral, Llama-2, Mixtral, GPT-3.5, GPT-4, and Claude-2.1. This dataset is chosen to evaluate the generalization capability of our approach, ensuring its robust performance across diverse text and summary conditions.
% \cmtOh{지환 작성 부탁}
% 1. 다양한 모델과 도메인이 있는 Unisumeval 썼다. 

\paragraph{Evaluation Metric}

% 다른 부분에서 언급되는거라 삭제
% We assess the quality of text summaries from three key perspectives: \textbf{faithfulness}, measured by the proportion of factually accurate summary sentences; \textbf{completeness}, reflecting the proportion of key facts covered; and \textbf{conciseness}, indicating the proportion of summary sentences that align with key facts. 

% 키팩트는 휴먼 키팩트가 이미 있음.
% For automated evaluation, key facts are extracted automatically from the reference summaries of each source dataset.

We evaluate different refinement pipelines for three dimensions. To achieve this, we FineSurE using GPT-4o \cite{song2024finesure}. We adapt the FineSure to align with test dataset's error taxonomy, reducing the number of error types from nine to five. We computed the revised summary scores on three dimensions via automatic evaluation using the key facts within the dataset. We provide results by other model and G-Eval, tailored to three dimensions and in Appendix \ref{sec:appendix-other-evaluation}



\section{Main Results}
\label{sec:main-result}

\subsection{Comparision of Previous Pipelines}

Table \ref{tab:exp1-add} presents a comparative analysis between prior refinements, which are P1 focusing solely on faithfulness, and \algname{}. 
\algname{} demonstrates improvements across all dimensions without sacrificing performance in any dimensions. \textbf{In contrast, while previous pipelines achieved substantial gains in faithfulness, they suffer from an alignment tax in completeness}—a cost that was similarly observed during training \cite{song2024learning}. These results suggest that such trade-offs persist throughout the refinement process.

% This enhancement can be attributed to the synergistic effect arising from the integration of feedback across diverse dimensions. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[t]
\begin{center}
\footnotesize
\begin{tabular}{|L{1.6cm} |X{1.4cm} X{1.48cm} X{1.4cm}|} 
\toprule
Config. & Faith. & Comp. & Conc. \\ \midrule
% Before  & 78.0 & 46.4 & 76.4 \\

ACUEval & 80.8\textsuperscript{*} {\color{ForestGreen}\textbf{\scriptsize{(+2.8)}}} & 43.8\textsuperscript{*}{\color{BrickRed}\textbf{\scriptsize{(-2.6)}}} & 
81.9\textsuperscript{*}{\color{ForestGreen}\textbf{\scriptsize{(+5.5)}}} \\  

DCR  & 
81.2\textsuperscript{*}{\color{ForestGreen}\textbf{\scriptsize{(+3.2)}}} &
42.8\textsuperscript{*}{\color{BrickRed}\textbf{\scriptsize{(-3.6)}}} & 
76.7 {\color{ForestGreen}\textbf{\scriptsize{(+0.3)}}} \\

% C4 & 80.1\textsuperscript{*}  {\color{ForestGreen}\textbf{\scriptsize{(+2.1)}}} & 56.0\textsuperscript{*}  {\color{ForestGreen}\textbf{\scriptsize{(+9.6)}}} & \textbf{83.6\textsuperscript{*}}{\color{ForestGreen}\textbf{\scriptsize{(+7.2)}}} \\ 

% \algname{}  & \textbf{82.7\textsuperscript{*} } {\color{ForestGreen}\textbf{\scriptsize{(+4.7)}}} & \textbf{60.0\textsuperscript{*} } {\color{ForestGreen}\textbf{\scriptsize{(+13.6)}}} & 83.4\textsuperscript{*}{\color{ForestGreen}\textbf{\scriptsize{(+7.0)}}} \\ 

\algname{}& 
82.7\textsuperscript{*}{\color{ForestGreen}\textbf{\scriptsize{(+4.7)}}} & 60.0\textsuperscript{*} {\color{ForestGreen}\textbf{\scriptsize{(+13.6)}}} & 83.4\textsuperscript{*}{\color{ForestGreen}\textbf{\scriptsize{(+7.0)}}} \\ 

\algname{}\textsubscript{QwQ} & 
\textbf{83.8\textsuperscript{*} }{\color{ForestGreen}\textbf{\scriptsize{(+5.8)}}} & \textbf{61.5\textsuperscript{*} }{\color{ForestGreen}\textbf{\scriptsize{(+15.1)}}} & \textbf{83.8}\textsuperscript{*}{\color{ForestGreen}\textbf{\scriptsize{(+7.4)}}} \\ 

% \algname{} & \textbf{82.7\textsuperscript{*} } {\color{ForestGreen}\textbf{\scriptsize{(+4.7)}}} & \textbf{60.0\textsuperscript{*} } {\color{ForestGreen}\textbf{\scriptsize{(+13.6)}}} & 83.4\textsuperscript{*}{\color{ForestGreen}\textbf{\scriptsize{(+7.0)}}} \\ 
\bottomrule
\end{tabular}
\end{center}
\vspace*{-0.4cm}
\caption{Comparison with the previous refinement pipeline, which focused solely on faithfulness, by using automated evaluation to assess the revised summary on faithfulness, completeness, and conciseness. \textsuperscript{*} denotes statistically significant difference with p < 0.05 according to a paired bootstrap test.}
\label{tab:exp1-add}
\vspace*{-0.4cm}
\end{table}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%% Refine Performance Results %%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[t]
\begin{center}
\footnotesize
\begin{tabular}{ |X{1.12cm} |X{0.9cm} |X{1.57cm} |X{1.75cm} |X{1.27cm} |X{1.38cm} X{1.42cm} X{1.38cm} |X{1.38cm}|} \toprule
ID & Dim. & Feedback & Refinement & Reason & Faith. & Comp. & Conc. & Avg. \\ \midrule
\multicolumn{5}{|c|}{Before Refine} & 78.0 & 46.4 & 76.4 & 66.9 \\ \midrule
P1 & Faith. & Independent & Sequential & Receptive & 80.7\textsuperscript{*}{\color{ForestGreen}\textbf{\scriptsize{(+2.7)}}} & 45.9 {\color{BrickRed}\textbf{\scriptsize{(-0.5)}}} & 80.4\textsuperscript{*}{\color{ForestGreen}\textbf{\scriptsize{(+4.0)}}} & 69.0\textsuperscript{*}{\color{ForestGreen}\textbf{\scriptsize{(+2.1)}}} \\
P1 & Comp. & Independent & Sequential & Receptive & 80.4\textsuperscript{*}{\color{ForestGreen}\textbf{\scriptsize{(+2.4)}}} & \textbf{62.0\textsuperscript{*}}{\color{ForestGreen}\textbf{\scriptsize{(+15.6)}}} & 79.0\textsuperscript{*}{\color{ForestGreen}\textbf{\scriptsize{(+2.6)}}} & 73.8\textsuperscript{*}{\color{ForestGreen}\textbf{\scriptsize{(+6.9)}}} \\
P1 & Conc. & Independent & Sequential & Receptive & 76.7 {\color{BrickRed}\textbf{\scriptsize{(-1.3)}}} & 44.2\textsuperscript{*}{\color{BrickRed}\textbf{\scriptsize{(-2.2)}}} & \textbf{86.3\textsuperscript{*}}{\color{ForestGreen}\textbf{\scriptsize{(+9.9)}}} & 69.1\textsuperscript{*}{\color{ForestGreen}\textbf{\scriptsize{(+2.2)}}} \\\midrule
P2 & Multi & Independent & Sequential & Receptive & 78.4\textsuperscript{*}{\color{ForestGreen}\textbf{\scriptsize{(+0.4)}}} & 51.5\textsuperscript{*}{\color{ForestGreen}\textbf{\scriptsize{(+5.1)}}} & 84.8\textsuperscript{*}{\color{ForestGreen}\textbf{\scriptsize{(+8.4)}}} & 71.6\textsuperscript{*}{\color{ForestGreen}\textbf{\scriptsize{(+4.7)}}} \\\midrule
P3 & Multi & Dependent & Sequential & Receptive & 78.9 {\color{ForestGreen}\textbf{\scriptsize{(+0.9)}}} & 53.2\textsuperscript{*}{\color{ForestGreen}\textbf{\scriptsize{(+6.8)}}} & 80.0\textsuperscript{*}{\color{ForestGreen}\textbf{\scriptsize{(+3.6)}}} & 70.7\textsuperscript{*}{\color{ForestGreen}\textbf{\scriptsize{(+3.8)}}} \\\midrule
P4 & Multi & Dependent & Simultaneous & Receptive & 80.1\textsuperscript{*}{\color{ForestGreen}\textbf{\scriptsize{(+2.1)}}} & 56.0\textsuperscript{*}{\color{ForestGreen}\textbf{\scriptsize{(+9.6)}}} & 83.6\textsuperscript{*}{\color{ForestGreen}\textbf{\scriptsize{(+7.2)}}} & 73.2\textsuperscript{*}{\color{ForestGreen}\textbf{\scriptsize{(+6.3)}}} \\\midrule 

\algname{} & Multi & Dependent & Simultaneous & Reflective & \textbf{82.7\textsuperscript{*}}{\color{ForestGreen}\textbf{\scriptsize{(+4.7)}}} & 60.0\textsuperscript{*}{\color{ForestGreen}\textbf{\scriptsize{(+13.6)}}} & 83.4\textsuperscript{*}{\color{ForestGreen}\textbf{\scriptsize{(+7.0)}}} & \textbf{75.3\textsuperscript{*}}{\color{ForestGreen}\textbf{\scriptsize{(+8.4)}}} \\


% RF\textsubscript{w.o FT} & Multi & Dependent & Simultaneous & Reflective & \textbf{81.0\textsuperscript{*}}{\color{ForestGreen}\textbf{\scriptsize{(+4.7)}}} & 56.1\textsuperscript{*}{\color{ForestGreen}\textbf{\scriptsize{(+13.6)}}} & 79.8\textsuperscript{*}{\color{ForestGreen}\textbf{\scriptsize{(+7.0)}}} & \textbf{75.3\textsuperscript{*}}{\color{ForestGreen}\textbf{\scriptsize{(+8.4)}}} \\


\bottomrule
\end{tabular}
\end{center}
\vspace*{-0.4cm}
\caption{Automated evaluation results of revised summary on faithfulness, completeness and conciseness across across refinement pipeline.  The best score are marked in bold.}
\label{tab:exp1}
\vspace*{-0.45cm}
\end{table*}

% \textsuperscript{*} denotes statistically significant difference with p < 0.05 according to a paired bootstrap test.



%%%%%%%%%%%%%% Table for noisy feedback %%%%%%%%
\begin{table}[t]
\setlength{\tabcolsep}{5pt}
\renewcommand{\arraystretch}{1}
\begin{center}
\footnotesize
\begin{tabular}{ |l|c c|c c|c c| }
\toprule
\multirow{2}{*}{ID} & \multicolumn{2}{c|}{Faith.} & \multicolumn{2}{c|}{Comp.} & \multicolumn{2}{c|}{Conc.} \\ \cmidrule{2-7}
 & High & Low & High & Low  & High  & Low \\ \midrule
Before. & \multicolumn{2}{c|}{78.0} & \multicolumn{2}{c|}{46.4} & \multicolumn{2}{c|}{76.4} \\ \midrule
DCR & 81.9\textsuperscript{*} & 81.2\textsuperscript{*} & 48.0\textsuperscript{*} & 42.8\textsuperscript{*} & 80.1\textsuperscript{*} & 76.7 \\ 
P1\textsubscript{Faith} & 82.2\textsuperscript{*} & 80.7\textsuperscript{*} & 47.1\textsuperscript{*} & 45.9 & 79.7\textsuperscript{*} & 80.4\textsuperscript{*} \\ 
P1\textsubscript{Comp} & 82.7\textsuperscript{*} & 80.4\textsuperscript{*} & \textbf{66.2\textsuperscript{*}} & \textbf{62.0\textsuperscript{*}} & 80.9\textsuperscript{*} & 79.0\textsuperscript{*} \\ 
P1\textsubscript{Conc} & 78.9 & 76.7 & 45.5\textsuperscript{*} & 44.2\textsuperscript{*} & \textbf{86.9\textsuperscript{*}} & \textbf{86.3\textsuperscript{*}} \\ 
P4 & 
83.3\textsuperscript{*} & 80.1\textsuperscript{*} & 60.0\textsuperscript{*} & 56.0\textsuperscript{*} & 84.8\textsuperscript{*} & 83.6\textsuperscript{*} \\ 

% C5 wo FT & \textbf{84.6\textsuperscript{*}} & \textbf{82.7\textsuperscript{*}} & 62.5\textsuperscript{*} & 60.0\textsuperscript{*} & 84.0\textsuperscript{*} & 83.4\textsuperscript{*} \\ 

\algname{}& \textbf{84.6\textsuperscript{*}} & \textbf{82.7\textsuperscript{*}} & 62.5\textsuperscript{*} & 60.0\textsuperscript{*} & 84.0\textsuperscript{*} & 83.4\textsuperscript{*} \\ \bottomrule


\end{tabular}
\end{center}
\vspace*{-0.4cm}
\caption{Comparison of refinement pipelines under low- and high-quality feedback. "Before." indicates the score of summary based on automated evaluation before refinement.}
\label{tab:exp3}
\vspace*{-0.6cm}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Insights on Multi-Dimensional Refinement}

We conduct experiments across diverse environments to identify the optimal settings across multi-dimensions by investigating our RQs. 

\subsubsection{RQ1: The Impact of Each Configuration} We compare five pipelines, which use the "reason+refine" module, to analyze the impact of each configuration. Table \ref{tab:exp1} presents the revised summary quality across five refinement pipelines, evaluating performance before and after refinement.

Single dimension refinement (P1) achieve the sufficient gains in the targeted dimension; however, such improvement can come at the cost of other dimensions. While P1\textsubscript{Faith} and P1\textsubscript{Conc} yields the competent improvement in faithfulness and conciseness, respectively, they introduce trade-offs in multi-dimensional refinement. \textbf{Managing these trade-offs is strongly influenced by dependency on multi-feedback.} Comparing P2 and P3, P2 maximizes conciseness but suffers from the lowest completeness, whereas P3 achieves a more balanced improvement by considering dependencies.

Above all, the sequential strategies underperform compared to the simultaneous one, as their composite score ("Avg.") is lower. Given the trade-off between conciseness and other dimensions observed in P1\textsubscript{Conc}, it can be attributed to an order bias favoring conciseness as the last dimension. \textbf{In the simultaneous setting, reflective reasoning is a pivotal role in managing trade-offs and handling noisy feedback.} \algname{} demonstrates a notable improvement over P4, with an increase of 2.6 in faithfulness and 4.0 in completeness, while maintaining conciseness with only a minor difference of 0.2.



% %%%%%%%%%%%% 구버전
% \subsubsection{RQ1: The Impact of Each Configuration}
% To analyze the impact of configuration within the multi-dimensions, we compare five pipelines incorporating the "reason+refine" module. Table \ref{tab:exp1} presents the revised summary quality across five refinement pipelines, evaluating performance before and after refinement.

% \textbf{While single dimension refinement (P1) achieve the sufficient gains in the targeted dimension, such improvement can come at the cost of other dimensions.} P1\textsubscript{Faith} and P1\textsubscript{Conc} yields the competent improvement in faithfulness and conciseness, but they introduces a decline in other dimensions, unlike multi-dimension refinement, which benefits all aspects. Furthermore, \textbf{recognizing the dependency on feedback plays a crucial role in handling trade-off.} Comparing P2 and P3, although P2 achieves the highest conciseness, it exhibits the lowest completeness among the multi-dimensional pipelines. Conversely, P3 demonstrates a more balanced improvement by accounting for dependencies on multi-dimensions.

% \textbf{Abobe all, the sequential strategy exhibits lower composite score ("Avg.") compared to the simultaneous one.} Given the trade-off between conciseness and other dimensions observed in P1\textsubscript{Conc}, it can be attributed to an order bias favoring conciseness as the last dimension—a bias that is further amplified in the independent configuration. Conversely, the simultaneous strategy more effectively handles dependencies on multi-dimensions and thereby mitigates this trade-off. 

% \textbf{In the simultaneous setting, where dependencies across dimensions are strongest, reflective reasoning is a pivotal role in managing trade-offs and handling noisy feedback.} \algname{} demonstrates a notable improvement over P4, with an increase of 2.6 in faithfulness and 4.0 in completeness, while maintaining conciseness with only a minor difference of 0.2.

% %%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%
% e observe that reflective reasoning enables backtracking when trade-offs arise during refinement while selectively integrating only valid feedback, rather than passively incorporating all feedback. Appendix \ref{sec:appendix-reasoning-case-study} provides a detailed qualitative analysis of receptive and reflective reasoning.

%%%%%%%%%%%%%%%%%%%%%%%%%


\subsubsection{RQ2 : Robustness against Feedback Quality}

Next, we compare the refinement performance achieved using low-quality detection labels with that obtained using high-quality labels. We exclude ACUEval from this comparison because it does not use sentence-level labels. We generate feedback using LLaMA 3.1 70B-instruct, assuming the 70B model produces high-quality feedback with more exact label based on its evaluation of agreement with humans in Appendix \ref{sec:appendix-feedback-quality}. Table~\ref{tab:exp3} presents results of the automated evaluation when transitioning from high- to low-quality feedback. 

\algname{} robustly handles both high- and low-quality feedback. For example, compared to the next-best multi-dimensional method (P4), \algname{} shows smaller drops in faithfulness (1.9 vs. 3.2), completeness (2.5 vs. 4.0), and conciseness (0.6 vs. 1.2). Even with low-quality feedback, \algname{} outperforms P1\textsubscript{Faith}—which focuses solely on faithfulness—even under high-quality conditions. In contrast, single-dimensional pipelines suffer in their targeted areas, and noise in one dimension can negatively impact others. \textbf{This is likely to show cross-dimensional effect, with noisy feedback in one dimension potentially impairing performance in others.} While DCR and P1\textsubscript{Faith} maintain completeness under clean feedback, their scores drop when noise is introduced. \textbf{These results demonstrate the value of reflective reasoning in mitigating noise by validating incorrect feedback. }

% \textbf{\algname{} consistently maintains robust performance under both high- and low-quality feedback conditions.} Specifically, when comparing P4, which is next best choice for multi-dimension as seen in Table \ref{tab:exp1}, \algname{} exhibits differences of 1.9, 2.5, and 0.6 in $\triangle$Faith, $\triangle$Comp, and $\triangle$Conc, respectively, whereas P4 shows markedly larger degradations of 3.2, 4.0, and 1.2 in three dimensions. This highlights the potential of reflective reasoning to filter out noisy feedback. 

% Notably, even under low-quality feedback, \algname{} outperforms P1\textsubscript{Faith}—designed focusing on refining only faithfulness—even under high-quality feedback. In contrast, each single-dimensional pipeline exhibits distinct performance drops within its respective dimensions, indicating that all dimensions possess inherent sensitivities to noise. \textbf{Moreover, the results are like to show cross-dimensional effect, with noisy feedback in one dimension potentially impairing performance in others.} Although both DCR and P1\textsubscript{Faith} maintain completeness relative to original summary under relatively clean feedback, completeness fall below the scores observed before revised under noise. 

%%%%%%%%%%%%%% Table for order bias (수정후) with Avg. Composite Score %%%%%%%%%%%%%%
\begin{table*}[]
\footnotesize
\begin{center}
\begin{tabular}{|X{1cm} |X{0.4cm} X{0.4cm} X{0.4cm}| X{0.4cm} X{0.4cm} X{0.4cm} | X{0.4cm} X{0.4cm} X{0.4cm} | X{0.4cm} X{0.4cm} X{0.4cm} | X{0.4cm} X{0.4cm} X{0.4cm} | X{1.5cm} |}
\toprule
\multirow{3}{*}{\!\!\!Id\!\!\!} &
\multicolumn{3}{c}{\!\!\!Trial 1\!\!\!} &
\multicolumn{3}{c}{\!\!\!Trial 2\!\!\!} & 
\multicolumn{3}{c}{\!\!\!Trial 3\!\!\!} & 
\multicolumn{3}{c}{\!\!\!Trial 4\!\!\!} & 
\multicolumn{3}{|c|}{\multirow{2}{*}{\!\!\!Max--Min\!\!\!}} & 
\multirow{3}{*}{\makecell{Average\\Composite\\Score}} \\
\cmidrule(lr){2-13} 
& \multicolumn{3}{c}{\!\!\!Random\!\!\!} &
\multicolumn{3}{c}{\!\!\!Last--Faith\!\!\!} &
\multicolumn{3}{c}{\!\!\!Last--Comp\!\!\!} &
\multicolumn{3}{c}{\!\!\!Last--Conc\!\!\!} &
\multicolumn{3}{|c|}{} & \\
\cmidrule(lr){2-16}
& \!\!\!FA\!\!\! & \!\!\!CM\!\!\! & \!\!\!CN\!\!\! & \!\!\!FA\!\!\! & \!\!\!CM\!\!\! & \!\!\!CN\!\!\! & \!\!\!FA\!\!\! & \!\!\!CM\!\!\! & \!\!\!CN\!\!\! & \!\!\!FA\!\!\! & \!\!\!CM\!\!\! & \!\!\!CN\!\!\! & \!\!\!FA\!\!\! & \!\!\!CM\!\!\! & \!\!\!CN\!\!\! & \\
\midrule
\!\!\!P2\!\!\! &
\!\!\!80.8\!\!\! & \!\!\!59.1\!\!\! & \!\!\!\textbf{85.3}\!\!\! & 
\!\!\!80.9\!\!\! & \!\!\!59.0\!\!\! & \!\!\!\textbf{85.0}\!\!\! & 
\!\!\!81.1\!\!\! & \!\!\!\textbf{63.2}\!\!\! & \!\!\!83.9\!\!\! & 
\!\!\!79.6\!\!\! & \!\!\!55.3\!\!\! & \!\!\!\textbf{85.1}\!\!\! & 
\!\!\!1.5\!\!\! & \!\!\!7.9\!\!\! & \!\!\!1.4\!\!\! & 74.9 \\
\!\!\!P3\!\!\! & 
\!\!\!80.7\!\!\! & \!\!\!59.3\!\!\! & \!\!\!82.8\!\!\! & 
\!\!\!80.8\!\!\! & \!\!\!57.7\!\!\! & \!\!\!82.5\!\!\! & 
\!\!\!80.4\!\!\! & \!\!\!62.5\!\!\! & \!\!\!82.4\!\!\! & 
\!\!\!79.5\!\!\! & \!\!\!58.4\!\!\! & \!\!\!83.0\!\!\! & 
\!\!\!1.3\!\!\! & \!\!\!4.8\!\!\! & \!\!\!0.6\!\!\! & 74.2 \\
\!\!\!P4\!\!\! & 
\!\!\!83.8\!\!\! & \!\!\!61.3\!\!\! & \!\!\!85.1\!\!\! & 
\!\!\!82.9\!\!\! & \!\!\!60.6\!\!\! & \!\!\!84.9\!\!\! & 
\!\!\!\textbf{83.6}\!\!\! & \!\!\!60.7\!\!\! & \!\!\!83.8\!\!\! & 
\!\!\!81.9\!\!\! & \!\!\!59.8\!\!\! & \!\!\!84.8\!\!\! & 
\!\!\!1.9\!\!\! & \!\!\!1.5\!\!\! & \!\!\!1.3\!\!\! & 76.1 \\ \midrule
\multicolumn{1}{|l|}{\!\!\!\algname{}\!\!\!} & 
\!\!\!\textbf{84.2}\!\!\! & \!\!\!\textbf{62.9}\!\!\! & \!\!\!84.2\!\!\! & 
\!\!\!\textbf{83.6}\!\!\! & \!\!\!\textbf{62.6}\!\!\! & \!\!\!84.6\!\!\! & 
\!\!\!83.4\!\!\! & \!\!\!62.4\!\!\! & \!\!\!\textbf{84.5}\!\!\! & 
\!\!\!\textbf{84.3}\!\!\! & \!\!\!\textbf{62.9}\!\!\! & \!\!\!84.4\!\!\! & 
\!\!\!\textbf{0.9}\!\!\! & \!\!\!\textbf{0.5}\!\!\! & \!\!\!\textbf{0.4}\!\!\! & \textbf{77.0} \\

\multicolumn{1}{|l|}{\!\!\!\algname{}(--)\!\!\!} & 
\!\!\!\textbf{84.2}\!\!\! & \!\!\!61.1\!\!\!& \!\!\!85.2\!\!\! & 
\!\!\!83.3\!\!\! & \!\!\!60.1\!\!\! & \!\!\!84.2\!\!\! & 
\!\!\!82.7\!\!\! & \!\!\!60.1\!\!\! & \!\!\!\textbf{84.5}\!\!\! & 
\!\!\!83.1\!\!\! & \!\!\!61.6\!\!\! & \!\!\!84.5\!\!\! & 
\!\!\!1.5\!\!\! & \!\!\!1.5\!\!\! & \!\!\!0.7\!\!\! & 76.3 \\


\bottomrule
\end{tabular}
\end{center}
\vspace*{-0.4cm}
\caption{Automated evaluation results of different multi-dimensional refinement pipelines across four trials. FA, CM, and CN denote faithfulness, completeness, and conciseness, respectively. “Last–” indicates that the corresponding dimension was fixed as the final in the refinement order. "Max–Min" denotes the difference between the highest and lowest values, with the optimal (smallest) value highlighted in bold. The average composite score computed as the mean of the average scores for three dimensions. \algname{}(--) denotes the fine-tuend model on datasets where dimension order is not shuffled.}
\label{tab:exp2}
\vspace*{-0.5cm}
\end{table*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% %%%%%%%%%%%%%% Table for order bias (수정전)%%%%%%%%
% \begin{table*}[]
% \footnotesize
% \begin{center}
% \begin{tabular}{|X{0.5cm} |X{0.35cm} X{0.35cm} X{0.35cm}| X{0.35cm} X{0.35cm} X{0.35cm} | X{0.35cm} X{0.35cm} X{0.35cm} | X{0.35cm} X{0.35cm} X{0.35cm} | X{1.5cm} X{1.5cm} X{1.5cm} |}
% \toprule
% \multirow{3}{*}{\!\!\!Id\!\!\!} & \multicolumn{3}{c}{\!\!\!Trial 1\!\!\!} & \multicolumn{3}{c}{\!\!\!Trial 2\!\!\!} & \multicolumn{3}{c}{\!\!\!Trial 3\!\!\!} & \multicolumn{3}{c}{\!\!\!Trial 4\!\!\!} & \multicolumn{3}{|c|}{\multirow{2}{*}{\!\!\!Average\!\!\!}} \\
% \cmidrule(lr){2-13}
%                     & \multicolumn{3}{c}{\!\!\!Random\!\!\!} & \multicolumn{3}{c}{\!\!\!Last--Faith\!\!\!} & \multicolumn{3}{c}{\!\!\!Last--Comp\!\!\!} & \multicolumn{3}{c}{\!\!\!Last--Conc\!\!\!} & \multicolumn{3}{|c|}{} \\
% \cmidrule(lr){2-16}
%                     & \!\!\!FA\!\!\! & \!\!\!CM\!\!\! & \!\!\!CN\!\!\! & \!\!\!FA\!\!\! & \!\!\!CM\!\!\! & \!\!\!CN\!\!\! & \!\!\!FA\!\!\! & \!\!\!CM\!\!\! & \!\!\!CN\!\!\! & \!\!\!FA\!\!\! & \!\!\!CM\!\!\! & \!\!\!CN\!\!\! & \!\!\!FA\!\!\! & \!\!\!CM\!\!\! & \!\!\!CN\!\!\! \\
% \midrule
% \!\!\!P2\!\!\! &
% \!\!\!80.8\!\!\! & \!\!\!59.1\!\!\! & \!\!\!\textbf{85.3}\!\!\! & 
% \!\!\!80.9\!\!\! & \!\!\!59.0\!\!\! & \!\!\!\textbf{85.0}\!\!\! & 
% \!\!\!81.1\!\!\! & \!\!\!\textbf{63.2}\!\!\! & \!\!\!83.9\!\!\! & 
% \!\!\!79.6\!\!\! & \!\!\!55.3\!\!\! & \!\!\!\textbf{85.1}\!\!\! & 
% \!\!\!81.0 (±0.15)\!\!\! & \!\!\!59.3 (±2.99)\!\!\! & \!\!\!85.0 (±0.84)\!\!\! \\
% \!\!\!P3\!\!\! & 
% \!\!\!80.7\!\!\! & \!\!\!59.3\!\!\! & \!\!\!82.8\!\!\! & 
% \!\!\!80.8\!\!\! & \!\!\!57.7\!\!\! & \!\!\!82.5\!\!\! & 
% \!\!\!80.4\!\!\! & \!\!\!62.5\!\!\! & \!\!\!82.4\!\!\! & 
% \!\!\!79.5\!\!\! & \!\!\!58.4\!\!\! & \!\!\!83.0\!\!\! & 
% \!\!\!80.5 (±0.32)\!\!\! & \!\!\!59.6 (±2.05)\!\!\! & \!\!\!82.8 (±0.40)\!\!\! \\
% \!\!\!P4\!\!\! & 
% \!\!\!83.8\!\!\! & \!\!\!61.3\!\!\! & \!\!\!85.1\!\!\! & 
% \!\!\!82.9\!\!\! & \!\!\!60.6\!\!\! & \!\!\!84.9\!\!\! & \!\!\!\textbf{83.6}\!\!\! & \!\!\!60.7\!\!\! & \!\!\!83.8\!\!\! & \!\!\!81.9\!\!\! & \!\!\!59.8\!\!\! & \!\!\!84.8\!\!\! & 
% \!\!\!83.6 (±0.45)\!\!\! & \!\!\!60.7 (±0.42)\!\!\! & \!\!\!84.9 (±0.76)\!\!\! \\
% \!\!\!R3F\!\!\! & 
% \!\!\!\textbf{84.2}\!\!\! & \!\!\!\textbf{62.9}\!\!\! & \!\!\!84.2\!\!\! & \!\!\!\textbf{83.6}\!\!\! & \!\!\!\textbf{62.6}\!\!\! & \!\!\!84.6\!\!\! & \!\!\!83.4\!\!\! & \!\!\!62.4\!\!\! & \!\!\!\textbf{84.5}\!\!\! & \!\!\!\textbf{84.3}\!\!\! & \!\!\!\textbf{62.9}\!\!\! & \!\!\!84.4\!\!\! & \!\!\!83.9 (±0.44)\!\!\! & \!\!\!62.7 (±0.24)\!\!\! & \!\!\!84.4 (±0.17)\!\!\! \\
% \bottomrule
% \end{tabular}
% \end{center}
% \vspace*{-0.4cm}
% \caption{Automated evaluation results of different multi-dimensional refinement pipeline across multiple trials. FA, CM, and CN denote faithfulness, completeness, and conciseness, respectively. "Last--" indicates that the corresponding dimension was fixed as the final in the refinement order. R3F refer to \algname{}.}
% \label{tab:exp2}
% \vspace*{-0.5cm}
% \end{table*}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\subsubsection{RQ3 : Robustness against Ordering Bias}
Lastly, we conducted four trials with shuffled orders to assess the impact of ordering bias. In first trials, each data point is assigned a random permutation of three dimensions. For Trials 2-4, we fix the final position of each dimension, while the remaining positions is randomized. For details on the distribution of orders, See Appendix \ref{sec:appendix-experiment-detail-order}. We use high-quality labels, which are almost free of noise, ensuring that our analysis focuses on the impact of order bias. we also compare with \algname{}--, which was fine-tuned on a non-shuffled dataset, to examine the effects of shuffling on ordering bias. Table \ref{tab:exp2} summarizes the performance of different refinement pipelines across four trials.

\algname{} shows enhanced stability owing to its refinement strategy and training method. In sequential pipelines P2 and P3, completeness varies widely (Max-Min values of 7.9 and 4.8, respectively). \textbf{This variability likely stems from order bias—later dimensions overly influence refinement, as evidenced by P2’s superior scores on its final dimension.} Moreover, independent style in P2 exacerbates this fluctuations. By contrast, simultaneous strategies avoid such order bias. P4 and \algname{}, which are simultaneous refinement, achieves overall low variances. \textbf{Notably, shuffling the dimension order in train data mitigates ordering bias, resulting in both improved overall performance and reduced variance.} Consequently, \algname{} achieves minimal variance, with max–min differences of 0.9 in faithfulness, 0.5 in completeness, and 0.4 in conciseness.completeness, and 0.4 in conciseness).


% \algname{} demonstrates greater stability in automated evaluation results due to its refinement strategies and training method. A comparison between sequential and simultaneous strategies reveals key differences in robustness. sequential strategies such as P2 and P3 exhibit higher variance in completeness, with fluctuations reaching 
% "Max–Min" values of 7.9 and 4.8, respectively. \textbf{This variability likely stems from order bias: later dimensions in the sequential pipeline disproportionately influence refinement, overshadowing earlier dimensions.} This is evidenced by P2’s superior scores corresponding the last-ordered dimension in "Last-Comp" and "Last-Conc." Additionally, independent feedback mechanisms, as seen in P2, strengthen variability due to the lack of dependency-aware adjustments across dimensions.

% In contrast, \textbf{simultaneous strategies do not exhibit order bias stemming from the dimension's position in the prompt, indicating their robustness against order-related biases.} Notably, \algname{}, which employs a simultaneous refienment for multi-dimensional refinement, facilitates a more stable refinement. \algname{} exhibits the lowest variance across all dimensions, with a "Max–Min" values of 0.9, 0.5, and 0.4 in faithfulness, completeness, and conciseness, respectively. This stability can be attributed to the elimination of order bias by shuffling the order of dimensions. 
%%%%%%%%%%% 예전에 쓴 거 %%%%%%%%%%%%%%%

% The reasoning approach also plays a crucial role in performance stability. Reflective reasoning (C5) yields the overall stable results, especially completeness and conciseness, while maintaining competitive scores. This highlights the advantage of reflective reasoning enables models to balance competing quality criteria more effectively
%%%%%%%%%%% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% \vspace{-0.1cm}
\section{Additional Experiment For Reflective Feedback Reasnoning}
% \vspace{-0.1cm}
We conduct an in-depth investigation into the impact of reflective reasoning on the multi-dimensional refinement. We compare the performance of reflective reasoning against receptive one (P4), both distilled from the same teacher model. We use identical data construction process except the prompt design; we remove the guidelines intended to filter out noise and backtracking to adjust trade-off. Consequently, the final reasoning data by P4 comprises approximately 5K samples. For a fair comparison, we fine-tune both P4 and \algname{} using only the 4K \texttt{<doc, summary, feedback>} triplets present in both datasets. Appendix \ref{sec:appendix-additional-experiment} provides detailed statistics for each reasoning dataset. Table~\ref{tab:additonal-study1} summarizes the automated evaluation results of four reasoning settings.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table}[t]
\setlength{\tabcolsep}{2pt}
\renewcommand{\arraystretch}{1}
\begin{center}
\footnotesize
\begin{tabular}{|l|l|c c|c c|c c|}
\toprule
\multirow{2}{*}{Model.} & \multirow{2}{*}{ID} & \multicolumn{2}{c|}{Faith.} & \multicolumn{2}{c|}{Comp.} & \multicolumn{2}{c|}{Conc.} \\ \cmidrule{3-8}
 &  & High & Low & High & Low & High & Low \\ \midrule
\multirow{4}{*}{L3.1 8B} & C4                
& 83.3\textsuperscript{*} & 80.1\textsuperscript{*} & 60.0\textsuperscript{*} & 56.0\textsuperscript{*} & 84.8\textsuperscript{*} & 83.6\textsuperscript{*} \\ 

 & C4\textsubscript{FT}  & 82.0\textsuperscript{*} & 81.2\textsuperscript{*} & 56.6\textsuperscript{*} & 54.2\textsuperscript{*} & 82.7\textsuperscript{*} & 81.8\textsuperscript{*} \\ 
 & \algname{}\textsubscript{4k}  & 83.3\textsuperscript{*} & 81.6\textsuperscript{*} & 59.3\textsuperscript{*} & 56.0\textsuperscript{*} & 85.7\textsuperscript{*} & 85.2\textsuperscript{*} \\ 
 & \algname{}\textsubscript{8k}  & 84.6\textsuperscript{*} & 82.7\textsuperscript{*} & 62.5\textsuperscript{*} & 60.0\textsuperscript{*} & 84.0\textsuperscript{*} & 83.4\textsuperscript{*} \\ \bottomrule
\end{tabular}
\end{center}
\vspace*{-0.4cm}
\caption{Ablation on the reasoning style under low- and high-quality feedback. L3.1 8B represents LLaMA 3.1-8B-instruct. P4\textsubscript{FT} indicates that P4 was fine-tuned with 4K data. 4K and 8K refer to training data size.}
\label{tab:additonal-study1}
\vspace*{-0.5cm}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



P4\textsubscript{FT} model with 4K data exhibits low variance between high- and low-quality feedback (0.8, 2.4, and 0.9 across dimensions), yet its performance under high-quality conditions deteriorates relative to SFT—likely due to the lack of explicit goal and critique guidelines such as best summaries and factual error types, leading to over-rejection of feedback. Moreover, while the P5 model trained on 4K data shows robustness, training on 8K data significantly enhances performance while maintaining low variance across feedback qualities. These results highlight the importance of both carefully crafted reasoning guidelines and large data volumes for effectively balancing evaluative dimensions and boosting reasoning capabilities, consistent with prior work \cite{xu2025redstar}.


% \paragraph{Selection of Reasoning Models} Both the reasoning model and the student model C4\textsubscript{FT} and C5 exhibit a notable robusteness to noise. This indicates that the reasoning model appears capable of validating noisy feedback rather than merely receptive to feedback itself. This is evidenced by the consistently reduced variance observed between high- and low-quality feedback across student model and teacher model.
    
% Comparing P4\textsubscript{FT} and P5 with 4K data, the P4\textsubscript{FT} model shows low variance between high- and low-quality conditions, with 0.8, 2.4, and 0.9 across three dimensions. However, its performance under high-quality feedback declines before SFT, likely due to the absence of guideline—such as best summaries or factual error types—for effective critique. As a result, the model may overly reject feedback, limiting performance gains even under high-quality feedback conditions. These findings underscore the need for carefully crafted reasoning guidelines that effectively balance multiple evaluative dimensions. While the P5 with 4K data model exhibits robustness on feedback, its performance improvement is marginal compared to that of the P5 with 8K data. As the dataset size increases, performance gains become more pronounced while the low variance between high- and low-quality feedback is maintained. These findings underscore that large data volumes are crucial for enhancing reasoning capabilities, which is consistent with prior work \cite{xu2025redstar}.


% 1. Reasoning 모델 자체가 noisy에 강건한 특성을 가지고 있음. 즉 단순히 피드백에 receptive한게 아니라 noise를 validate할 수 있는 능력이 있음. configuration에 상관없이 High와 Low에서의 편차가 전반적으로 적어진 것을 확인할 수 있음

% 2. 그러나 단순히 noise에 대해 refute하는 능력은 reasoning guideline을 세밀하게 설정하는 것이 필요함. 단순히 C4에서 distillation하는 것은 너무 많이 refute하여 성능이 high에서도 크게 오르지않는 반면, C5에서는 high에서 gain을 확실히 얻고 있음. 이는 데이터 사이즈를 크게할수록 gain은 올라가면서 high와 low에서는 편차가 작아지는데, trade-off를 잘 컨트롤하는 방법을 learning하는 것의 중요성을 나타낸다고 볼 수 있음. 

\label{sec:additional-study}


% 공간 부족하여 보류 (실험도 애매하게 나옴)
% \section{Additional Experiment}
% \label{sec:additional-result}

% \subsection{Analysis of Reasoning}
% Noisy를 Reject 정말 하는지 Case study

% \subsection{Refinement on good summary (가제)}
% 1. 좋은 모델 써머리 고칠 수 있는지?

